Hybrid Cinematography: Previsualizing and Managing Hallucination Risk in Generative Video Reshooting

On a film set, the camera move is committed during a take. Generative video reshooting lets filmmakers change it afterward, but may require hallucinating unrecorded content, a gap sometimes discovered only after leaving the set. We present Hybrid Cinematography, a workflow that bridges physical capture and generative reshooting to manage hallucination risk while filmmakers can still act on it. Using an editable 3D shot plan and a proxy of the take, our previsualization evaluates hallucination risk in real time. Seeing where the take lacks support, filmmakers can iteratively adjust the plan, explore moves that balance capture and generation, shoot guided pickups, or knowingly accept hallucination. We demonstrate the workflow through a mobile augmented reality application for on-set planning, capture, and review, and an offline pipeline for existing video. A study with experienced filmmakers reveals how previsualizing risk informs camera decisions and exposes tensions between creative intent and generative hallucination.

==> macros/NotesAndEditsMacros.tex <==

\makeatletter
\@ifundefined{ifsubmit}{%
  \newif\ifsubmit
  \submittrue
}{}
\makeatother

\definecolor{ad_color}{rgb}{0,0.1,1.0}   %
\definecolor{nt_color}{rgb}{0,0.4,0.2}   %
\definecolor{ss_color}{RGB}{170,80,0}    %
\definecolor{nw_color}{RGB}{110,60,140}  %

\definecolor{mathbrace_color}{rgb}{0.2,0.5,1.0}

\makeatletter
\@ifundefined{germansharps}{%
  \let\germansharps\ss
}{}
\makeatother

\providecommand{\ad}[1]{#1}
\providecommand{\nt}[1]{#1}
\providecommand{\nw}[1]{#1}
\makeatletter
\@ifundefined{adblock}{\newenvironment{adblock}{}{}}{}
\@ifundefined{ntblock}{\newenvironment{ntblock}{}{}}{}
\@ifundefined{ssblock}{\newenvironment{ssblock}{}{}}{}
\@ifundefined{nwblock}{\newenvironment{nwblock}{}{}}{}
\makeatother

\ifsubmit
  \renewcommand{\ad}[1]{#1}
  \renewcommand{\nt}[1]{#1}
  \renewcommand{\ss}[1]{#1}
  \renewcommand{\nw}[1]{#1}
  \renewenvironment{adblock}{}{}
  \renewenvironment{ntblock}{}{}
  \renewenvironment{ssblock}{}{}
  \renewenvironment{nwblock}{}{}
\else
  \renewcommand{\ad}[1]{\textcolor{ad_color}{#1}}
  \renewcommand{\nt}[1]{\textcolor{nt_color}{#1}}
  \renewcommand{\ss}[1]{\textcolor{ss_color}{#1}}
  \renewcommand{\nw}[1]{\textcolor{nw_color}{#1}}
  \renewenvironment{adblock}{\color{ad_color}}{}
  \renewenvironment{ntblock}{\color{nt_color}}{}
  \renewenvironment{ssblock}{\color{ss_color}}{}
  \renewenvironment{nwblock}{\color{nw_color}}{}
\fi

